Mixture-based Feature Space Learning for Few-shot Image Classification

We introduce Mixture-based Feature Space Learning (MixtFSL) for obtaining a rich and robust feature representation in the context of few-shot image classification. Previous works have proposed to model each base class either with a single point or with a mixture model by relying on offline clustering algorithms. In contrast, we propose to model base classes with mixture models by simultaneously training the feature extractor and learning the mixture model parameters in an online manner. This results in a richer and more discriminative feature space which can be employed to classify novel examples from very few samples. Two main stages are proposed to train the MixtFSL model. First, the multimodal mixtures for each base class and the feature extractor parameters are learned using a combination of two loss functions. Second, the resulting network and mixture models are progressively refined through a leader-follower learning procedure, which uses the current estimate as a "target" network. This target network is used to make a consistent assignment of instances to mixture components, which increases performance and stabilizes training. The effectiveness of our end-to-end feature space learning approach is demonstrated with extensive experiments on four standard datasets and four backbones. Notably, we demonstrate that when we combine our robust representation with recent alignment-based approaches, we achieve new state-of-the-art results in the inductive setting, with an absolute accuracy for 5-shot classification of 82.45 on miniImageNet, 88.20 with tieredImageNet, and 60.70 in FC100 using the ResNet-12 backbone.

==> sec_associativeAlignment.tex <==
\section{Fast alignment without forgetting}
\label{sec:alignment} 


\todo{here, we will discuss the our new version of centroid alignment with cos similarity, new concatenated base-novel classification layer which do not have the forgetting problem }

\todo{here, we can add a figure and algorithm side by side}

\onecolumn
\begin{figure*}[!t] 
\begin{minipage}[t]{8.8cm}
  \ \\ 
     \begin{algorithm}[H]
    \SetAlgoLined
        \textbf{Input:} pre-trained model $c(f(\cdot|{\theta})|\mathbf{W})$, 
        novel class $\mathcal{X}^n$, related base set $\mathcal{X}^{rb}$.\\
        \textbf{Output:} fine-tuned $c(f(\cdot|{\theta})|\mathbf{W})$. \\ 
        \While{not done}
        {
        \small
            $\widetilde{\mathcal{X}}^n \leftarrow \text{sample a batch from } \mathcal{X}^n$ \\
            $\widetilde{\mathcal{X}}^{rb} \leftarrow \text{sample a batch from } \mathcal{X}^{rb}$  \\ 
            \ \\
            evaluate $\mathcal{L}_\mathrm{ca}(\widetilde{\mathcal{X}}^{n},\widetilde{\mathcal{X}}^{rb})$;  $\theta \leftarrow \theta - \eta_\mathrm{ca} \nabla_{\theta} \mathcal{L}_\mathrm{ca}(\widetilde{\mathcal{X}}^{n},\widetilde{\mathcal{X}}^{rb})$\\[0.5em]
    
            evaluate $\mathcal{L}_\mathrm{clf}(\widetilde{\mathcal{X}}^{rb})$; 
            $\mathbf{W} \leftarrow \mathbf{W} - \eta_\mathrm{clf} \nabla_{\mathbf{W}} \mathcal{L}_\mathrm{clf}(\widetilde{\mathcal{X}}^{rb})$\\ 
            evaluate $\mathcal{L}_\mathrm{clf}(\widetilde{\mathcal{X}}^{n})$;    $\mathbf{W} \leftarrow \mathbf{W} - \eta_\mathrm{clf} \nabla_{\mathbf{W}} \mathcal{L}_\mathrm{clf}(\widetilde{\mathcal{X}}^{n})$ 
            $\theta \leftarrow \theta - \eta_\mathrm{clf} \nabla_{\theta} \mathcal{L}_\mathrm{clf}(\widetilde{\mathcal{X}}^{n})$ \\ 
        }
        \caption{Centroid alignment without forgetting}
        \label{alg:centroid}
    \end{algorithm}
\end{minipage}%
~~
\begin{minipage}[t]{8.5cm} \ \\
  \centering
  \includegraphics[width=.7\linewidth]{figures_plots/cartoons/architecture_novel_90_v2.pdf}
        \caption{Schematic overview of our centroid alignment without forgetting. The feature learner $f(\cdot|\theta)$ takes a batch of examples from base examples \todo{wotk on the caption} $\mathbf{x}^n$ and an example related base $\mathbf{x}_i^{rb}$. A Euclidean centroid based alignment loss $\mathcal{L}_\mathrm{ca}$ (red arrow) aligns the encoded $\mathbf{x}_i^n$ and $\mathbf{x}^{rb}_i$. Blue arrows represent classification loss $\mathcal{L}_\mathrm{clf}$.} 
        \label{fig:centroid-align} 
\end{minipage} 
\end{figure*}
\twocolumn
  



==> table_FineGrain_CrossDomain.tex <==
\begin{table}[t]
\renewcommand{\tabcolsep}{2pt}
\centering
\caption{
Camparition of our MixtFSL and alignment (MixtFSL-Align.) using CUB in 5-way classification. Here, bold/blue is best/second best, and $\pm$ indicates the 95\% confidence intervals over 600 episodes.} 
\begin{tabular}{rlccc}  
        \toprule  
        & \textbf{Method}   
        & \textbf{\small Backbone} 
        & \textbf{1-shot}  
        & \textbf{5-shot}    
        \\  
        \midrule   
        & Robust-20~\cite{dvornik2019diversity}   
                & {\small RN-18}
                & 58.67\scriptsize{ $\pm$0.65}     & 75.62\scriptsize{ $\pm$0.48}     
                    \\      
                      
                & RelationNet$^\ddag$~\cite{sung2018learning}      
                    & {\small RN-18} 
                    & 67.59\scriptsize{ $\pm$1.02}             & 82.75\scriptsize{ $\pm$0.58}     
                     \\
                     
                & MAML~\cite{finn2017model}    
                    & {\small RN-18}
                    &  68.42\scriptsize{ $\pm$1.07}           & 83.47\scriptsize{ $\pm$0.62} 
                    \\
                    
                & RelationNet~\cite{sung2018learning}    
                    & {\small RN-18} 
                    & 68.58\scriptsize{ $\pm$0.94}           & 84.05\scriptsize{ $\pm$0.56} 
                    \\
                    
                & MatchingNet~\cite{vinyals2016matching}   
                    & {\small RN-18}
                    & 73.49\scriptsize{ $\pm$0.89}           & 84.45\scriptsize{ $\pm$0.58} 
                    \\
                    
                & ProtoNet$^{\ddag}$~\cite{snell2017prototypical}    
                    & {\small RN-18}
                    & {\color{blue}71.88}\scriptsize{ $\pm$0.91}             & 86.64\scriptsize{ $\pm$0.51} 
                    \\
                    
                & Arcmax~\cite{Afrasiyabi_2020_ECCV} 
                    & {\small RN-18}
                    & 71.37\scriptsize{ $\pm$0.86}      & 85.74\scriptsize{ $\pm$0.49}
                    \\
                    
                & Cent. Align.~\cite{Afrasiyabi_2020_ECCV} 
                    & {\small RN-18}
                    & {\color{blue}74.22}\scriptsize{ $\pm$1.09}      & \textbf{88.65}\scriptsize{ $\pm$0.55}
                    \\*[.5em]
         
                              
                    & MixtFSL (ours)  
                    & {\small RN-18}
                    & {\color{blue}73.94} \scriptsize{ $\pm$1.05}      & {\color{blue}86.01}\scriptsize{ $\pm$0.52}     
                    \\  
                & MixtFSL-Align. (ours) 
                    & {\small RN-18} 
                    & \textbf{74.29} \scriptsize{ $\pm$0.87}      &{\color{blue}87.76}\scriptsize{ $\pm$0.63}  
                    \\ 
            \cmidrule(lr){2-5}         
                
                        
                & GNN-LFT~\cite{tseng2020cross}        %{\color{red}RN-10}
                    & {\small RN-10}   
                     & 51.51\scriptsize{ $\pm$0.80}     & 73.11\scriptsize{ $\pm$0.68}     
                     \\
         
                & Neg-cosine~\cite{Bin_2020_ECCV_margin_matter}  %\todo{ECCV2020: read this}   
                    & {\small RN-12} 
                    & 72.66    \scriptsize{ $\pm$0.85}           & \textbf{89.40}\scriptsize{ $\pm$0.43} 
                    \\
                     
                & Arcmax~\cite{Afrasiyabi_2020_ECCV}$^{\dag}$       
                    & {\small RN-12} 
                    & 72.14    \scriptsize{ $\pm$0.59}           & 86.47\scriptsize{ $\pm$0.59} 
                    \\*[.5em]
                      
            %\cmidrule(lr){2-5}           
                & MixtFSL (ours) 
                    & {\small RN-12} 
                    & {\color{blue}{76.01}}  \scriptsize{ $\pm$0.80}      & 88.21\scriptsize{ $\pm$0.45}  
                    \\ 
                    
                & MixtFSL-Align. (ours) 
                    & {\small RN-12} 
                    & \textbf{76.65}  \scriptsize{ $\pm$0.71}      & {\color{blue}{89.26}}\scriptsize{ $\pm$0.65}  
                    \\ 
    
  
        \midrule       
    \end{tabular}  \\
    \quad  $^*$ implementation is from~\cite{tang2020long} \quad   $^{\dag}$ our implementation \quad    
    $^{\ddag}$ implementation from~\cite{chen2019closer}
    \label{tab:baselines}
\end{table}














\begin{table}[!t]
\centering
\renewcommand{\tabcolsep}{2pt}
\caption {Cross-domain results from miniImageNet to CUB in 1-shot, 5-shot, 10-shot scenarios using a ResNet-18 backbone.Here, bold/blue is best/second best.} 
    \begin{tabular}{clcc} %c
        \toprule
        & Method     & 1-shot     & 5-shot        %& 10-shot 
        \\    
        \midrule
        %\multirow{3}{*}{\rotatebox{90}{meta-l.}}
	    & ProtoNet$^\ddag$~\cite{wang2018low}               & --                           & 62.02\scriptsize{ $\pm$ 0.70}      
	    %& -- 
	    \\   
	    
	    & MAML$^\ddag$~\cite{finn2018probabilistic}         & --                           & 51.34\scriptsize{ $\pm$ 0.72}      
	    %& --
	    \\   
	    
	    & RelationNet$^\ddag$~\cite{sung2018learning}       & --                           & 57.71\scriptsize{ $\pm$ 0.73}      
	    %& -- 
	    \\  
	    
	    & Diverse 20~\cite{dvornik2019diversity} & --                                      & 66.17\scriptsize{ $\pm$ 0.73}   
	    %& --
	    \\  
  
        & cosmax$^{\dag}$~\cite{chen2019closer}  & 43.06\scriptsize{ $\pm$ 1.01}           & 64.38\scriptsize{ $\pm$ 0.86}             
        \\
	   
	    & Arcmax~\cite{Afrasiyabi_2020_ECCV}         & 45.60\scriptsize{ $\pm$ 0.94}            & 64.93\scriptsize{ $\pm$ 0.95}               
	    \\
	    
	    
	    & Neg-cosine~\cite{Bin_2020_ECCV_margin_matter}              & --                           & 67.03  \scriptsize{ $\pm$ 0.76}      
	    %& -- 
	    \\   
	    
	    & Cent.Align.~\cite{Afrasiyabi_2020_ECCV}                  
	    & \textbf{47.25}\scriptsize{ $\pm$ 0.76}    & \textbf{72.37}\scriptsize{ $\pm$ 0.89}      
	    \\*[.5em] 
	    
	     
        
        & MixtFSL (ours)         
        & {\color{blue}44.56}\scriptsize{ $\pm$ 1.06}      %still running ...
        & {\color{blue}68.77}\scriptsize{ $\pm$ 0.93}           %& 00.00\scriptsize{ $\pm$ 00.00}    
        \\ 
	    \bottomrule
    \end{tabular} \\  
    $^\ddag$ implementation from \cite{chen2019closer} 
    \label{tab:cross-domain} 
\end{table}
























\begin{table}[t]
\renewcommand{\tabcolsep}{2pt}
\centering
\caption{
Camparition of our MixtFSL and alignment (MixtFSL-Align.) using CUB in 5-way classification. Here, bold/blue is best/second best, and $\pm$ indicates the 95\% confidence intervals over 600 episodes.} 
\begin{tabular}{rlccc}  
        \toprule   
        & \textbf{Method} %& \textbf{\small Backbone} 
        & \textbf{1-shot}   & \textbf{5-shot}   &\textbf{5-shot}  \\
        &  & & &MI $\xrightarrow{} $ CUB  \\ 
        \midrule          
            \multirow{6}{*}{\rotatebox{90}{ResNet-12}}             
                & GNN-LFT~\cite{tseng2020cross}        %{\color{red}RN-10}
                    %& {\small RN-10}   
                     & 51.51\scriptsize{ $\pm$0.80}     & 73.11\scriptsize{ $\pm$0.68}     
                     &--  
                     \\
         
                & Neg-cosine~\cite{Bin_2020_ECCV_margin_matter}  %\todo{ECCV2020: read this}   
                    %& {\small RN-12} 
                    & 72.66    \scriptsize{ $\pm$0.85}           & \textbf{89.40}\scriptsize{ $\pm$0.43} 
                    &-- 
                    \\
                     
                & Arcmax~\cite{Afrasiyabi_2020_ECCV}$^{\dag}$       
                    %& {\small RN-12} 
                    & 72.14    \scriptsize{ $\pm$0.59}           & 86.47\scriptsize{ $\pm$0.59} 
                    &--  
                    \\
                    
                & Neg-cosine~\cite{Bin_2020_ECCV_margin_matter}   
                    %& {\small RN-12} 
                    & 72.14    \scriptsize{ $\pm$0.59}           & 86.47\scriptsize{ $\pm$0.59} 
                    &--  
                    \\*[.5em]
                      
            %\cmidrule(lr){2-5}           
                & MixtFSL (ours) 
                    %& {\small RN-12} 
                    & \textbf{76.01}\scriptsize{ $\pm$0.80}      & {\color{blue}88.21}\scriptsize{ $\pm$0.45}  
                    &--  
                    \\ 
                    
                %& MixtFSL-Align. (ours) 
                %    & {\small RN-12} 
                %    & \textbf{76.65}  \scriptsize{ $\pm$0.71}      & {\color{blue}{89.26}}\scriptsize{ $\pm$0.65}  
                %    & 00.00\scriptsize{ $\pm$0.00}
                %    \\  
        
        \midrule  
        %&  & & & MI $\xrightarrow{} $ CUB \\
        %& \textbf{Method} %& \textbf{\small Backbone} 
        %& \textbf{1-shot}   & \textbf{5-shot} & \textbf{5-shot} \\
        %\midrule  
        \multirow{9}{*}{\rotatebox{90}{ResNet-18}}
                & Robust-20~\cite{dvornik2019diversity}   
                %& {\small RN-18}
                & 58.67\scriptsize{ $\pm$0.65}     & 75.62\scriptsize{ $\pm$0.48}  
                & --
                    \\      
                      
                & RelationNet$^\ddag$~\cite{sung2018learning}      
                    %& {\small RN-18} 
                    & 67.59\scriptsize{ $\pm$1.02}             & 82.75\scriptsize{ $\pm$0.58} 
                    & 57.71\scriptsize{ $\pm$0.73}
                     \\
                     
                & MAML$^\ddag$~\cite{finn2017model}    
                    %& {\small RN-18}
                    & 68.42\scriptsize{ $\pm$1.07}           & 83.47\scriptsize{ $\pm$0.62} 
                    & 51.34\scriptsize{ $\pm$0.72}
                    \\
                    
                %& RelationNet~\cite{sung2018learning}    
                    %& {\small RN-18} 
                %    & 68.58\scriptsize{ $\pm$0.94}           & 84.05\scriptsize{ $\pm$0.56} 
                %    & 00.00\scriptsize{ $\pm$0.00}
                %    \\
                    
                & MatchingNet$^\ddag$~\cite{vinyals2016matching}   
                    %& {\small RN-18}
                    & 73.49\scriptsize{ $\pm$0.89}           & 84.45\scriptsize{ $\pm$0.58} 
                    & 53.07\scriptsize{ $\pm$0.74}
                    \\
                    
                & ProtoNet$^{\ddag}$~\cite{snell2017prototypical}    
                    %& {\small RN-18}
                    & 71.88\scriptsize{ $\pm$0.91}             & \textbf{86.64}\scriptsize{ $\pm$0.51} 
                    & 62.02\scriptsize{ $\pm$0.70}
                    \\
                    
                & Baseline++~\cite{chen2019closer} 
                    %& {\small RN-18}
                    & 67.02\scriptsize{ $\pm$0.90}      &  83.58\scriptsize{ $\pm$0.54}
                    & 64.38\scriptsize{ $\pm$0.86}
                    \\ 
                
                & Arcmax~\cite{Afrasiyabi_2020_ECCV} 
                    %& {\small RN-18}
                    & 71.37\scriptsize{ $\pm$0.86}      & 85.74\scriptsize{ $\pm$0.49}
                    & 64.93\scriptsize{ $\pm$0.95}
                    \\
                    
                & Neg-cosine~\cite{Bin_2020_ECCV_margin_matter}  %\todo{ECCV2020: read this}   
                    %& {\small RN-12} 
                    & --           & -- 
                    & {\color{blue}67.03}\scriptsize{ $\pm$0.76}
                    \\*[.5em]
                    
                %& Cent. Align.~\cite{Afrasiyabi_2020_ECCV} 
                %    & {\small RN-18}
                %    & {\color{blue}74.22}\scriptsize{ $\pm$1.09}      & \textbf{88.65}\scriptsize{ $\pm$0.55}
                %    \\
                
         
                    
                     
            %\cmidrule(lr){2-5}           
                    & MixtFSL (ours)  
                    %& {\small RN-18}
                    & \textbf{73.94}\scriptsize{ $\pm$1.05}      & {\color{blue}86.01}\scriptsize{ $\pm$0.52} 
                    & \textbf{68.77}\scriptsize{ $\pm$0.93}
                    \\  
                    
                %& MixtFSL-Align. (ours) 
                %    & {\small RN-18} 
                %    & \textbf{74.29} \scriptsize{ $\pm$0.87}      &\textbf{87.76}\scriptsize{ $\pm$0.63}  
                %    & 00.00\scriptsize{ $\pm$0.00}
                %    \\  
        \midrule       
    \end{tabular}  \\
    \quad  $^*$ implementation is from \cite{tang2020long} \quad   $^{\dag}$ our implementation \quad    
    \label{tab:baselines}
\end{table}












































\begin{table}[t]
\renewcommand{\tabcolsep}{2pt}
\centering
\caption{
Camparition of our MixtFSL and alignment (MixtFSL-Align.) using CUB in 5-way classification. Here, bold/blue is best/second best, and $\pm$ indicates the 95\% confidence intervals over 600 episodes.} 
\begin{tabular}{rlccc}  
        \toprule  
        & \textbf{Method}   
        & \textbf{\small Backbone} 
        & \textbf{1-shot}  
        & \textbf{5-shot}    
        \\  
        \midrule   
        & Robust-20~\cite{dvornik2019diversity}   
                & {\small RN-18}
                & 58.67\scriptsize{ $\pm$0.65}     & 75.62\scriptsize{ $\pm$0.48}     
                    \\      
                      
                & RelationNet$^\ddag$~\cite{sung2018learning}      
                    & {\small RN-18} 
                    & 67.59\scriptsize{ $\pm$1.02}             & 82.75\scriptsize{ $\pm$0.58}     
                     \\
                     
                & MAML~\cite{finn2017model}    
                    & {\small RN-18}
                    &  68.42\scriptsize{ $\pm$1.07}           & 83.47\scriptsize{ $\pm$0.62} 
                    \\
                    
                & RelationNet~\cite{sung2018learning}    
                    & {\small RN-18} 
                    & 68.58\scriptsize{ $\pm$0.94}           & 84.05\scriptsize{ $\pm$0.56} 
                    \\
                    
                & MatchingNet~\cite{vinyals2016matching}   
                    & {\small RN-18}
                    & 73.49\scriptsize{ $\pm$0.89}           & 84.45\scriptsize{ $\pm$0.58} 
                    \\
                    
                & ProtoNet$^{\ddag}$~\cite{snell2017prototypical}    
                    & {\small RN-18}
                    & 71.88\scriptsize{ $\pm$0.91}             & {\color{blue}86.64}\scriptsize{ $\pm$0.51} 
                    \\
                    
                & Arcmax~\cite{Afrasiyabi_2020_ECCV} 
                    & {\small RN-18}
                    & 71.37\scriptsize{ $\pm$0.86}      & 85.74\scriptsize{ $\pm$0.49}
                    \\*[.5em]
                    
                %& Cent. Align.~\cite{Afrasiyabi_2020_ECCV} 
                %    & {\small RN-18}
                %    & {\color{blue}74.22}\scriptsize{ $\pm$1.09}      & \textbf{88.65}\scriptsize{ $\pm$0.55}
                %    \\
                
         
                    
                      
            %\cmidrule(lr){2-5}           
                    & MixtFSL (ours)  
                    & {\small RN-18}
                    & {\color{blue}73.94} \scriptsize{ $\pm$1.05}      & 86.01\scriptsize{ $\pm$0.52}     
                    \\  
                & MixtFSL-Align. (ours) 
                    & {\small RN-18} 
                    & \textbf{74.29} \scriptsize{ $\pm$0.87}      &\textbf{87.76}\scriptsize{ $\pm$0.63}  
                    \\ 
            \cmidrule(lr){2-5}        
            %\bottomrule    
        %\multirow{14}{*}{\rotatebox{90}{ResNet-12}} 
        
                
                        
                & GNN-LFT~\cite{tseng2020cross}        %{\color{red}RN-10}
                    & {\small RN-10}   
                     & 51.51\scriptsize{ $\pm$0.80}     & 73.11\scriptsize{ $\pm$0.68}     
                     \\
         
                & Neg-cosine~\cite{Bin_2020_ECCV_margin_matter}  %\todo{ECCV2020: read this}   
                    & {\small RN-12} 
                    & 72.66    \scriptsize{ $\pm$0.85}           & \textbf{89.40}\scriptsize{ $\pm$0.43} 
                    \\
                     
                & Arcmax~\cite{Afrasiyabi_2020_ECCV}$^{\dag}$       
                    & {\small RN-12} 
                    & 72.14    \scriptsize{ $\pm$0.59}           & 86.47\scriptsize{ $\pm$0.59} 
                    \\*[.5em]
                      
            %\cmidrule(lr){2-5}           
                & MixtFSL (ours) 
                    & {\small RN-12} 
                    & {\color{blue}{76.01}}  \scriptsize{ $\pm$0.80}      & 88.21\scriptsize{ $\pm$0.45}  
                    \\ 
                    
                & MixtFSL-Align. (ours) 
                    & {\small RN-12} 
                    & \textbf{76.65}  \scriptsize{ $\pm$0.71}      & {\color{blue}{89.26}}\scriptsize{ $\pm$0.65}  
                    \\ 
    
  
        \midrule       
    \end{tabular}  \\
    \quad  $^*$ implementation is from \cite{tang2020long} \quad   $^{\dag}$ our implementation \quad    
    \label{tab:baselines}
\end{table}
